Regularized Q-learning

Q-learning is widely used algorithm in reinforcement learning community. Under the lookup table setting, its convergence is well established. However, its behavior is known to be unstable with the linear function approximation case. This paper develops a new Q-learning algorithm that converges when linear function approximation is used. We prove that simply adding an appropriate regularization term ensures convergence of the algorithm. We prove its stability using a recent analysis tool based on switching system models. Moreover, we experimentally show that it converges in environments where Q-learning with linear function approximation has known to diverge. We also provide an error bound on the solution where the algorithm converges.

==> algorithm/algorithm.tex <==
 

==> existence_uniqueness/solution.tex <==
We prove the existence and uniqueness of the solution of projected bellman equation when the regularization term is added.

\begin{lemma}\label{equilibrium_point_uniqueness}
Let \begin{equation}\label{reg_solution}
    -(1+\eta)X^TDX\theta_e + \gamma X^TDP\Pi_{\pi_{X\theta_e}} X\theta_e + X^TDR =0
\end{equation}
Under \Cref{full_rank_assumption}, and \( \eta = \max (0,\max_{\pi_{\theta},i}\frac{\gamma d^T p_{\pi_{\theta}}(i|\cdot)}{2d_i}- \frac{2-\gamma}{2}+\epsilon)\), the equilirbrium point exists and it is unique.
\end{lemma}

\begin{proof}
By Brouwer's fixed point theorem the solution exists. Uniqueness follows from the global asymptotic stability of~\ref{original_ode_theta}.
% \begin{align}
%         -X^TDX\theta_e + \frac{\gamma }{(1+\eta)}X^TDP\Pi_{\pi_{X\theta_e}} X\theta_e + X^TD(\frac{1}{1+\eta}R) &= 0\\
% \end{align}
% This is projected bellman equation with discount factor \( \frac{\gamma}{1+\eta}\) and reward \(\frac{1}{1+\eta}R\). Projected bellman equation has unique solution.
\end{proof}

% \begin{lemma}[Bias of the Solution]

% \end{lemma}

==> preliminaries/ode_analysis.tex <==
% {\color{blue}[To save the space, we can move the ODE analysis and switching system sections to appendix, because we do not show the proofs in the main text, so the backgrounds are not essential ]}

% The dynamic system framework has been widely used to prove convergence of reinforcement learning algorithms, e.g.,~\citealt{sutton2009fast,maei2010toward,borkar2000ode,lee2019unified}. Especially,~\citealp{borkar2000ode} is one of the most widely used techniques to prove stability of stochastic approximation using O.D.E. analysis. Consider the following stochastic algorithm with a nonlinear mapping \(f: \R^n \rightarrow \R^n\):
% \begin{align}
%      &\theta_{k+1} = f(\theta_k) + m_k, \quad\label{eq:stochastic-algorithm}
% \end{align}
% where $m_k \in \R^n$ is an i.i.d. noise vector. For completeness, results in~\citealp{borkar2000ode} are briefly reviewed in the sequel. Under Assumption~\ref{borkar_meyn_assumption} given in~\Cref{app:asmp}, we now introduce Borkar and Meyn theorem below.
% \begin{lemma}[Borkar and Meyn theorem]\label{borkar_meyn_lemma}
%     Suppose that Assumption~\ref{borkar_meyn_assumption} in the ~\Cref{app:asmp} holds, and consider the stochastic algorithm in~(\ref{eq:stochastic-algorithm}). Then, for any initial \(\theta_0 \in \R^n \), \(\sup_{k\geq 0}||\theta_k|| < \infty \) with probability one. In addition , 
%     \( \theta_k \rightarrow \theta^e \) as \( k \rightarrow \infty \) with probability one, where \( f(\theta^e)=0 \).
% \end{lemma}

% The main idea of Borkar and Meyn theorem is as follows: iterations of a stochastic recursive algorithm follow the solution of its corresponding O.D.E. in the limit when the step-size satisfies the Robbins-Monro condition. Hence, by proving the asymptotic stability of the O.D.E., we can induce the convergence of the original algorithm. In this paper, we will use an O.D.E. model of Q-learning, which is expressed as a special nonlinear system called a switching system. In the sequel, basic concepts in switching system theory are briefly introduced.

% Using switching system analysis, \cite{lee2019unified} proved stability of Q-learning algorithms including asynchronous, averaging and linear function approximation. The assumption used in linear function approximation is weaker than \cite{melo2008analysis} but still quite restrictive.

